Unsupervised Understanding of Location and Illumination Changes in Egocentric Videos

Wearable cameras stand out as one of the most promising devices for the upcoming years, and as a consequence, the demand of computer algorithms to automatically understand the videos recorded with them is increasing quickly. An automatic understanding of these videos is not an easy task, and its mobile nature implies important challenges to be faced, such as the changing light conditions and the unrestricted locations recorded. This paper proposes an unsupervised strategy based on global features and manifold learning to endow wearable cameras with contextual information regarding the light conditions and the location captured. Results show that non-linear manifold methods can capture contextual patterns from global features without compromising large computational resources. The proposed strategy is used, as an application case, as a switching mechanism to improve the hand-detection problem in egocentric videos.

==> tables/confusionMatrixSOMRF_EDSH.tex <==

\begin{table}[h!]
    \scriptsize
    \setlength{\tabcolsep}{4pt} % General space between cols (6pt standard)
    \centering
    \caption{Confusion matrix of SOM and RF using the global HSV and the hand-crafted feature for the
location problem of UNIGE dataset. Values represent percentages.} \label{tab:confusionHSV}
%\begin{tabular}{rr|>{\centering}m{0.4cm}>{\centering}m{0.4cm}>{\centering}m{0.4cm}>{\centering}m{0.\toprule



\end{table}


==> tables/videoSegmentation.tex <==
\begin{table}[h!]
    \scriptsize
    \setlength{\tabcolsep}{4pt} % General space between cols (6pt standard)
    \centering
    \caption{Confusion matrix of SOM and RF using the global HSV and the hand-crafted feature for the
location problem of UNIGE dataset. Values represent percentages.} \label{tab:confusion}
%\begin{tabular}{rr|>{\centering}m{0.4cm}>{\centering}m{0.4cm}>{\centering}m{0.4cm}>{\centering}m{0.\toprule

\begin{tabular}{rr|rrrrr|rrrrr}
\toprule
     &      & \multicolumn{5}{c|}{SOM}          & \multicolumn{5}{c}{RF} \\
\midrule
     &      & \begin{sideways}Kitchen\end{sideways} & \begin{sideways}Office\end{sideways} & \begin{sideways}Bar\end{sideways} & \begin{sideways}Street\end{sideways} & \begin{sideways}Park\end{sideways} & \begin{sideways}Kitchen\end{sideways} & \begin{sideways}Office\end{sideways} & \begin{sideways}Bar\end{sideways} & \begin{sideways}Street\end{sideways} & \begin{sideways}Park\end{sideways} \\ \midrule
\multicolumn{1}{c}{\multirow{5}[0]{*}{\begin{sideways}Hand Crafted\end{sideways}}} & Kitchen & \textbf{98.4} & 0.0  & 0.3  & 0.0  & 1.2  & \textbf{97.8} & 0.3  & 0.0  & 0.0  & 1.9 \\
\multicolumn{1}{c}{} & Office & 0.0  & \textbf{94.6} & 0.4  & 0.0  & 5.1  & 0.4  & \textbf{86.6} & 1.1  & 0.0  & 12.0 \\
\multicolumn{1}{c}{} & Bar  & 0.0  & 0.0  & \textbf{99.7} & 0.0  & 0.3  & 0.0  & 0.0  & \textbf{99.7} & 0.3  & 0.0 \\
\multicolumn{1}{c}{} & Street & 0.4  & 0.0  & 1.8  & \textbf{97.8} & 0.0  & 0.0  & 0.0  & 1.5  & \textbf{96.7} & 1.8 \\
\multicolumn{1}{c}{} & Park & 1.3  & 1.3  & 0.4  & 0.4  & \textbf{96.7} & 2.1  & 2.1  & 0.0  & 0.0  & \textbf{95.8} \\
\bottomrule
\end{tabular}%


\end{table}


==> tables/videoSegmentationEDSH.tex <==
\begin{table}[h!]
    \footnotesize
    \setlength{\tabcolsep}{4pt} % General space between cols (6pt standard)
\centering
    \caption{General Comparison of the unsupervised outputs.} \label{tab:general}
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{rr|rrrrr}
\toprule
  &       & \begin{sideways}Kitchen\end{sideways} & \begin{sideways}Office\end{sideways} & \begin{sideways}Bar\end{sideways} & \begin{sideways}Street\end{sideways} & \begin{sideways}Park\end{sideways} \\
\midrule
\multicolumn{1}{c}{\multirow{5}[0]{*}{SOM_{20}}} & Kitchen & 0.9   &       &       &       &  \\
\multicolumn{1}{c}{}                             & Office  &       & 0.85  &       &       &  \\
\multicolumn{1}{c}{}                             & Bar     &       &       & 0.93  &       &  \\
\multicolumn{1}{c}{}                             & Street  &       &       &       & 0..91 &  \\
\multicolumn{1}{c}{}                             & Park    &       &       &       &       & 0.5 \\ \midrule
\multicolumn{1}{c}{\multirow{5}[0]{*}{SVM}}      & Kitchen & 0.9   &       &       &       &  \\
\multicolumn{1}{c}{}                             & Office  &       & 0.85  &       &       &  \\
\multicolumn{1}{c}{}                             & Bar     &       &       & 0.93  &       &  \\
\multicolumn{1}{c}{}                             & Street  &       &       &       & 0..91 &  \\
\multicolumn{1}{c}{}                             & Park    &       &       &       &       & 0.5 \\ \bottomrule
\end{tabular}%
\end{table}

